Exploiting social networks dynamics for P2P resource organisation

In this paper we present a formal description of PROSA, a P2P resource management system heavily inspired by social networks. Social networks have been deeply studied in the last two decades in order to understand how communities of people arise and grow. It is a widely known result that networks of social relationships usually evolves to small-worlds, i.e. networks where nodes are strongly connected to neighbours and separated from all other nodes by a small amount of hops. This work shows that algorithms implemented into PROSA allow to obtain an efficient small-world P2P network.

==> prosa.tex <==
\section{\thealg: A brief introduction}
\label{s:prosa}
As said above, \thealg{} is a P2P network based on social relationships.
More formally, we can model \thealg{} as a direct graph:
	\begin{equation}
	\label{equ:prosa}
	\thealg{} = (\mathcal{P}, \mathcal{L}, P_k, Label)
	\end{equation}

$\mathcal{P}$ denotes the set of peers (i.e. vertices), 
$\mathcal{L}$ is the set of links $l = (s, t)$ (i.e. edges), where $t$ is a neighbor of $s$. 
For link $l = (s, t)$, $s$ is the source peer and $t$ is the target peer. All links are directed.

In P2P networks the knowledge of a peer is represented by the resources it shares with other peers.
In \thealg{} the mapping  $P_k: \mathcal{P} \rightarrow \mathcal{C}$, associates peers with 
resources. For a given peer $s \in \mathcal{P}$, $P_k(s)$ is a compact description of 
the peer knowledge ($PK$ - {\em Peer Knowledge}).

Relationships among people are usually based on similarities in interests, culture, 
hobbies, knowledge and so on. Usually these kind of links evolve from simple
``acquaintance--links'' to what we called ``semantic--links''.
To implement this behaviour three types of links have been introduced: {\em Acquaintance--Link} ($AL$),
{\em Temporary Semantic--Link} ($TSL$) and {\em Full Semantic--Link} ($FSL$).
TSLs represent relationships based on a partial knowledge of a
peer. They are usually stronger than $AL$s and weaker than $FSL$s.

In \thealg, if a given link is a simple $AL$, it means that the source peer does not know 
anything about the target peer. 
If the link is a $FSL$, the source peer knows all of the target peer (i.e. it 
knows the $P_k (t), \;t \in \mathcal{P}$ is the target peer). Finally, if the link is a $TSL$, 
the peer does not know the full $P_k(t)$ of the linked peer, but
a {\em Temporary Peer Knowledge} ($TP_k$) is built based on the query 
received from the source peer in the past.
The different behaviour of a link is modeled with a 
labelling function $Label$: for a given
link $l = (s,t) \in L$, $Label(l)$ is a vector of two elements $[e, w]$: the former is the link 
label and the latter is a weight used to model what the source peer knows of the target peer; this is computed 
as follow:
\begin{itemize}
	\item if $e = AL \Rightarrow w = \emptyset$ 
	\item if $e = TSL \Rightarrow w = TPK$
	\item if $e = FSL \Rightarrow w = P_k(t)$ 
\end{itemize}
In the next two sections, we will give a brief description of how \thealg{} works.
A detailed description of \thealg{} can be foun in \cite{PROSA@COPS06}.

%\begin{figure}[!htbp]
%	\centering
%	\includegraphics[scale=0.42]{links}
%	\caption{Link types}
%	\label{fig:links}
%\end{figure}

\subsection{Peer Joining to \thealg{}}
The case of a node that wants to join an existing network is
similar to the birth of a child. At the beginning of his life a
child ``knows'' just a couple of people (his parents). A new peer
which wants to join, just searches other peers at random
and enstabilish an $AL$s whit some of them. 
These links are $AL$s because a new peer doesn't know anything about
its neighbors until he doesn't query them for resources. This
behaviour is  quite easy to understand: when a baby comes to
life he doesn't know anything about his parents. 
The \thealg{} peer joining procedure is represented in algorithm \ref{join}.

\begin{algorithm}[hbt]
\caption{\small {\bf JOIN:} Peer $s$ joining to $\thealg (\mathcal{P},\mathcal{L}, P_k, Label)$}
\label{join}
\begin{algorithmic}[1]
	\REQUIRE $\thealg (\mathcal{P}, \mathcal{L}, P_k, Label), Peer\:s$
	\STATE $\mathcal{RP} \leftarrow rnd (P, n)$ \COMMENT {Ramdomly selects $n$ peers of \thealg}
	\STATE $\mathcal{P} \leftarrow \mathcal{P} \cup s$ \COMMENT {Adds $s$ to set of peers}
	\STATE $\mathcal{L} \leftarrow \mathcal{L} \cup \{(s, t), \forall t \in \mathcal{RP}\}$ 
		   \COMMENT {Links $s$ with the randomly selected peers}
	\STATE $\forall t \in \mathcal{RP} \Rightarrow Label(p, q) \leftarrow [AL, \emptyset]$
			\COMMENT {Sets the previously added links as $AL$}
\end{algorithmic}
\end{algorithm}

\subsection{\thealg{} dynamics}
In order to show how \thealg{} works, we need to define a query message model. 
Each query message is a quadruple:
\begin{equation}
	Q_M = (qid, q, s, n_r)
\end{equation}

where $qid$ is a unique query identifier to ensure that a peer does not
respond to a query more then once; $q$ is the query;  $s \in P$ is the 
source peer and $n_r$ is the number of required results. 

\thealg dynamic behaviour is modeled by the algorithm \ref{search}.

\begin{algorithm}
\caption{\footnotesize{\bf ExecQuery:} query $q$ originating from peer $s$ executed on peer $cur$}
\label{search}
\begin{algorithmic}[1]
	\REQUIRE $\thealg(\mathcal{P}, \mathcal{L}, P_k, Label)$
	\REQUIRE $cur, prev  \in \mathcal{P}, \;qm \in QueryMessage$
	\STATE $Result \leftarrow \emptyset $
	\IF {$prev \neq \emptyset$}
		\STATE $UpdateLink (\thealg, cur, prev, q)$
	\ENDIF
	\STATE $(Result,numRes) \leftarrow ResourcesRelevance (\thealg{}, q, cur, n_r)$
	\IF {$numRes = 0$}
		\STATE $f \rightarrow SelectForwarder(\thealg, cur, q)$
		\IF {$f \neq \emptyset$}
			\STATE $ExecQuery (\thealg, f, cur, qm)$
		\ENDIF
	\ELSE
		\STATE $SendMessage (s, cur, Result)$
		\STATE $\mathcal{L} \leftarrow \mathcal{L} \cup (s, cur)$
		\STATE $Label (s, cur) \leftarrow [FSL, P_k(cur)]$
		\IF {$numRes < n_r$}
			\STATE \COMMENT {-- Semantic Flooding --}
			\FORALL {$t \in Neighborhood(cur)$}
				\STATE $rel \rightarrow PeerRelevance(P_{k}(t), q)$
				\IF {$rel > Threshold$}
					\STATE $qm \leftarrow (qid, q, s, n_r - numRes)$
					\STATE $ExecQuery (\thealg, t, cur, qm)$
				\ENDIF
			\ENDFOR
		\ENDIF
	\ENDIF
\end{algorithmic}
\end{algorithm}


\thealg dynamics is strictly related to
queries.  When a user ($s$) of \thealg requires a 
resource, he performs a query $q$ and specify a certain number of
results he wants to obtain $n_r$. This is equivalent to
call $ExecQuery (\thealg, s, \emptyset, n_r)$.

The first time $ExecQuery$ is called, $prev$ is equal to $\emptyset$ and this
prevents from the execution of instruction number $3$. The successive call 
of $ExecQuery$, i.e. when a peer receives a query forwarded by another peer, 
the function $UpdateLink$ is called. This function updates link between 
current peer $cur$ and the forwarding peer $prev$. If the requesting peer 
is an unknown peer, a new $TSL$ link to that peer is added having as weigth
a Temporary Peer ($TP_k$) built based on query. 
If the requesting peer is a $TSL$ for the
peer that receives the query, the corresponding TPV in the list is
updated. If the requesting peer is a $FSL$, no updates
are necessary.
	
The relevance of the
query with the resources hosted by the user's peer is first
evaluated (calling function $ResourcesRelevance$). If none of the
hosted resources has a sufficient relevance with the query, the
query has to be forwarded to another peer $f$. 
This peer is selected among $s$ neighbors by the function $SelectForwarder$, using
the following mechanism:
	
	\begin{itemize}
	\item[-]
	Peer $s$ computes the relevance between the query $q$ and the weight of each links
	connectiong $s$ with neighborhood. 
	\item[-]
	It selects the link with a higher relevance, if it exists, and
	forward the query message to it.
	\item[-]
	If the peer has neither $FSL$s nor $TSL$s, i.e. it has just $AL$s, the query
	message is forwarded to one link at random.
	\end{itemize}

In any case the query message is forwarded. This is represented in the algorithm \ref{search}
by means of a recursive call to $ExecQuery$.
	
If, instead, the peer hosts resources with sufficient relevance with respect to $q$, two cases are possible:
	\begin{itemize}
	\item[-]
	The peer has sufficient relevant documents to full-fill the
	request. In this case a result message is sent to the requesting
	peer and the query is no more forwarded.
	\item[-]
	The peer has a certain number of relevant documents, but they are
	not enough to full-fill the request (i.e. they are $< n_r$). 
	In this case a response message
	is sent to the requester peer, specifying the number of matching
	documents. The message query is
	forwarded to all the links in the neighborhood whose relevance with the query
	is higher than a given threshold (semantic flooding). The number of
	matched resources is subtracted from the number of total requested
	documents before forwarding. 
	\end{itemize}

	When the requesting peer receives a response message it presents the
	results to the user. If the user decides to download a certain
	resource from another peer, the requesting peer contacts the peer
	owning that resource and ask it for downloading. If download is
	accepted, the resource is sent to the requesting peer.




